Type-Based Unsourced Multiple Access

We generalize the type-based multiple access framework proposed by Mergen and Tong (2006) to the case of unsourced multiple access. In the proposed framework, each device tracks the state of a physical/digital process, quantizes this state, and communicates it to a common receiver through a shared channel in an uncoordinated manner. The receiver aims to estimate the type of the states, i.e., the set of states and their multiplicity in the sequence of states reported by all devices. We measure the type estimation error using the Wasserstein distance. Considering an example of multi-target position tracking, we show that type estimation can be performed effectively via approximate message passing. Furthermore, we determine the quantization resolution that minimizes the type estimation error by balancing quantization distortion and communication error.

==> figs/TV_WS_vs_Ma.tex <==
% \subcaptionbox{total variation}
% {
\begin{tikzpicture}
    \tikzstyle{every node}=[font=\footnotesize] 
    \begin{semilogyaxis}[
    scale only axis,
    width=2.7in,
    height=1.1in,
    grid=both,
    grid style={line width=.1pt, draw=gray!10},
    major grid style={line width=.2pt,draw=gray!50},
%scale only axis,
    xmin=5,
    xmax=50,
    extra x ticks={5},
    xlabel={number of targets, $\Ma$},
    ymin=1e-4,
    ymax=1,
    ytick = {1e-4,1e-3,1e-2,1e-1,1e0},
    ylabel={average total variation, $\dTV$},
     ylabel style = {xshift=-1mm},
     % legend pos=south east,
     legend style={draw=none,opacity=.9,at={(0.98,0.01)},anchor=south east},
    ]
        
       \addplot [color=red,line width=1.2pt]
        table[row sep=crcr]{%
            5.0e+00 4.2938e-04 \\ 
1.0e+01 1.5417e-03 \\ 
1.5e+01 3.4685e-03 \\ 
2.0e+01 5.3916e-03 \\ 
2.5e+01 6.9256e-03 \\ 
3.0e+01 8.4073e-03 \\ 
3.5e+01 9.5731e-03 \\ 
4.0e+01 1.0233e-02 \\ 
4.5e+01 1.0880e-02 \\ 
5.0e+01 1.1375e-02 \\
        };
        \addlegendentry{AMP};
        
  \addplot [color=black,dashed,line width=1.2pt]
        table[row sep=crcr]{%
           5.0e+00 3.7838e-04 \\ 
1.0e+01 1.5416e-03 \\ 
1.5e+01 3.5108e-03 \\ 
2.0e+01 5.6245e-03 \\ 
2.5e+01 8.7741e-03 \\ 
3.0e+01 1.7963e-02 \\ 
3.5e+01 4.0228e-02 \\ 
4.0e+01 7.8646e-02 \\ 
4.5e+01 1.6475e-01 \\ 
5.0e+01 2.0135e-01 \\ 
            };
        \addlegendentry{scalar AMP};

                \addplot [color=blue,mark=*,only marks]
        table[row sep=crcr]{%
            5.0e+00 4.2444e-04 \\ 
1.0e+01 1.7238e-03 \\ 
1.5e+01 3.6545e-03 \\ 
2.0e+01 5.4532e-03 \\ 
2.5e+01 6.5709e-03 \\ 
3.0e+01 7.7956e-03 \\ 
3.5e+01 8.5455e-03 \\ 
4.0e+01 1.0182e-02 \\ 
4.5e+01 1.0555e-02 \\ 
5.0e+01 1.1417e-02 \\ 
                };
        \addlegendentry{EP};

        \addplot [color=blue,mark=*,only marks]
        table[row sep=crcr]{%
            5.0e+00 3.3826e-03 \\ 
1.0e+01 1.1134e-02 \\ 
1.5e+01 2.3197e-02 \\ 
2.0e+01 3.9107e-02 \\ 
2.5e+01 6.4527e-02 \\ 
3.0e+01 7.2927e-02 \\ 
3.5e+01 9.4571e-02 \\ 
4.0e+01 1.1555e-01 \\ 
4.5e+01 1.8600e-01 \\ 
5.0e+01 2.0627e-01 \\ 
                };
        % \addlegendentry{EP};
        
       \addplot [color=red,line width=1.2pt,forget plot]
        table[row sep=crcr]{%
            5.0e+00 3.6752e-03 \\ 
1.0e+01 1.0407e-02 \\ 
1.5e+01 2.2995e-02 \\ 
2.0e+01 3.9571e-02 \\ 
2.5e+01 5.4520e-02 \\ 
3.0e+01 7.0676e-02 \\ 
3.5e+01 8.2486e-02 \\ 
4.0e+01 9.4352e-02 \\ 
4.5e+01 1.0388e-01 \\ 
5.0e+01 1.1263e-01 \\ 
        };
        % \addlegendentry{AMP};
        
  \addplot [color=black,dashed,line width=1.2pt, forget plot]
        table[row sep=crcr]{%
           5.0e+00 3.4610e-03 \\ 
1.0e+01 1.0378e-02 \\ 
1.5e+01 2.4877e-02 \\ 
2.0e+01 1.1351e-01 \\ 
2.5e+01 3.0327e-01 \\ 
3.0e+01 5.0991e-01 \\ 
3.5e+01 7.2020e-01 \\ 
4.0e+01 7.4202e-01 \\ 
4.5e+01 8.5617e-01 \\ 
5.0e+01 8.3923e-01 \\ 
            };
        % \addlegendentry{scalar AMP};

        \coordinate (Center) at (axis cs:15,2.1e-2);
   		\coordinate (Radius) at (axis cs:15.7,4e-2);
   		
   		\coordinate (Center2) at (axis cs:15,3.5e-3);
   		\coordinate (Radius2) at (axis cs:15.7,7e-3);

        \node[align = center] at (axis cs:16,1.4e-3) () {$\n = 500$};
        \node[align = center] at (axis cs:13,6e-2) () {$\n = 250$};
        
      \end{semilogyaxis}
      \pgfextractx{\rx}{\pgfpointdiff{\pgfpointanchor{Radius}{center}}{\pgfpointanchor{Center}{center}}}%
	\pgfextracty{\ry}{\pgfpointdiff{\pgfpointanchor{Radius}{center}}{\pgfpointanchor{Center}{center}}}%
	\draw (Center) ellipse [x radius = \rx, y radius = \ry]; 
	
	\pgfextractx{\rx}{\pgfpointdiff{\pgfpointanchor{Radius2}{center}}{\pgfpointanchor{Center2}{center}}}%
	\pgfextracty{\ry}{\pgfpointdiff{\pgfpointanchor{Radius2}{center}}{\pgfpointanchor{Center2}{center}}}%
	\draw (Center2) ellipse [x radius = \rx, y radius = \ry]; 
    \end{tikzpicture}
%     }
%     \subcaptionbox{Wasserstein distance}{
    
%     \begin{tikzpicture}
%     \tikzstyle{every node}=[font=\footnotesize] 
%     \begin{axis}[
%     scale only axis,
%     width=2.7in,
%     height=2in,
%     grid=both,
%     grid style={line width=.1pt, draw=gray!10},
%     major grid style={line width=.2pt,draw=gray!50},
% %scale only axis,
%     xmin=1,
%     xmax=50,
%     xlabel={number of targets, $\Ma$},
%     ymin=.2,
%     ymax=.25,
%     ylabel={average Wasserstein distance},
%      legend pos=north west,
%     ]
%   %      \addplot [color=gray!70,line width=2.5pt]
%   %       table[row sep=crcr]{%
%   %           1.000000000000000   0.192728752193278 \\
%   %  5.000000000000000   0.203499004643537 \\
%   % 10.000000000000000   0.203903736507754 \\
%   % 15.000000000000000   0.204112026940354 \\
%   % 20.000000000000000   0.204778161416724 \\
%   % 25.000000000000000   0.204842411757580 \\
%   % 30.000000000000000   0.204817225197270 \\
%   % 35.000000000000000   0.205044984566911 \\
%   % 40.000000000000000   0.204790238005981 \\
%   % 45.000000000000000   0.204934026102418 \\
%   % 50.000000000000000   0.204923443143492 \\
%   %           };
%   %       \addlegendentry{perfect com.};

%         \addplot [color=black,line width=1.2pt]
%         table[row sep=crcr]{%
%              5.0e+00 2.0413e-01 \\ 
% 1.0e+01 2.0543e-01 \\ 
% 1.5e+01 2.0647e-01 \\ 
% 2.0e+01 2.0615e-01 \\ 
% 2.5e+01 2.0553e-01 \\ 
% 3.0e+01 2.0601e-01 \\ 
% 3.5e+01 2.0588e-01 \\ 
% 4.0e+01 2.0597e-01 \\ 
% 4.5e+01 2.0585e-01 \\ 
% 5.0e+01 2.0508e-01 \\ 
%                 };
%         \addlegendentry{EP};
        
%         \addplot [color=blue,line width=1.2pt]
%         table[row sep=crcr]{%
%             5.0e+00 2.0135e-01 \\ 
% 1.0e+01 2.0474e-01 \\ 
% 1.5e+01 2.0491e-01 \\ 
% 2.0e+01 2.0598e-01 \\ 
% 2.5e+01 2.0537e-01 \\ 
% 3.0e+01 2.0594e-01 \\ 
% 3.5e+01 2.0627e-01 \\ 
% 4.0e+01 2.0498e-01 \\ 
% 4.5e+01 2.0622e-01 \\ 
% 5.0e+01 2.0501e-01 \\ 
%                 };
%         \addlegendentry{AMP};

%         \addplot [color=red,line width=1.2pt]
%         table[row sep=crcr]{%
%             5.0e+00 2.0246e-01 \\ 
% 1.0e+01 2.0439e-01 \\ 
% 1.5e+01 2.0395e-01 \\ 
% 2.0e+01 2.0531e-01 \\ 
% 2.5e+01 2.0519e-01 \\ 
% 3.0e+01 2.0583e-01 \\ 
% 3.5e+01 2.0536e-01 \\ 
% 4.0e+01 2.0624e-01 \\ 
% 4.5e+01 2.0509e-01 \\ 
% 5.0e+01 2.0369e-01 \\ 
%             };
%         \addlegendentry{scalar AMP};

%                 \addplot [color=black,line width=1.2pt,forget plot]
%         table[row sep=crcr]{%
%              5.0e+00 2.0428e-01 \\ 
% 1.0e+01 2.0737e-01 \\ 
% 1.5e+01 2.0842e-01 \\ 
% 2.0e+01 2.0959e-01 \\ 
% 2.5e+01 2.0782e-01 \\ 
% 3.0e+01 2.0910e-01 \\ 
% 3.5e+01 2.0945e-01 \\ 
% 4.0e+01 2.0621e-01 \\ 
% 4.5e+01 2.0903e-01 \\ 
% 5.0e+01 2.0453e-01 \\ 
%                 };
%         % \addlegendentry{EP};
        
%         \addplot [color=blue,line width=1.2pt,forget plot]
%         table[row sep=crcr]{%
%             5.0e+00 2.0381e-01 \\ 
% 1.0e+01 2.0736e-01 \\ 
% 1.5e+01 2.0831e-01 \\ 
% 2.0e+01 2.0916e-01 \\ 
% 2.5e+01 2.0940e-01 \\ 
% 3.0e+01 2.0868e-01 \\ 
% 3.5e+01 2.0998e-01 \\ 
% 4.0e+01 2.0974e-01 \\ 
% 4.5e+01 2.0793e-01 \\ 
% 5.0e+01 2.0883e-01 \\ 
%                 };
%         % \addlegendentry{AMP};

%         \addplot [color=red,line width=1.2pt, forget plot]
%         table[row sep=crcr]{%
%             5.0e+00 2.0429e-01 \\ 
% 1.0e+01 2.0735e-01 \\ 
% 1.5e+01 2.0730e-01 \\ 
% 2.0e+01 2.1243e-01 \\ 
% 2.5e+01 2.1580e-01 \\ 
% 3.0e+01 2.1921e-01 \\ 
% 3.5e+01 2.1576e-01 \\ 
% 4.0e+01 2.1150e-01 \\ 
% 4.5e+01 2.0839e-01 \\ 
% 5.0e+01 2.0462e-01 \\ 
%             };
%         % \addlegendentry{scalar AMP};
%       \end{axis}
%     \end{tikzpicture}
%     }

==> figs/TV_WS_vs_SNR.tex <==
% \subcaptionbox{total variation}[.5\textwidth][c]{
\begin{tikzpicture}
    \tikzstyle{every node}=[font=\footnotesize] 
    \begin{semilogyaxis}[
    scale only axis,
    width=2.7in,
    height=1.5in,
    grid=both,
    grid style={line width=.1pt, draw=gray!10},
    major grid style={line width=.2pt,draw=gray!50},
%scale only axis,
    xmin=-18,
    xmax=-4,
    xlabel={\gls{SNR}, $\power$ (dB)},
    ymin=1e-4,
    ymax=1e-1,
    ytick = {1e-5,1e-4,1e-3,1e-2,1e-1,1},
    ylabel={average total variation},
    ylabel style = {yshift=-1mm},
     legend pos=south west,
    ]
       \addplot [color=blue,line width=1.2pt]
        table[row sep=crcr]{%
          -2.0e+01 7.6473e-02 \\ 
-1.8e+01 5.0099e-02 \\ 
-1.6e+01 3.3092e-02 \\ 
-1.4e+01 2.0372e-02 \\ 
-1.2e+01 1.0769e-02 \\ 
-1.0e+01 5.3100e-03 \\ 
-8.0e+00 4.1015e-03 \\ 
-6.0e+00 2.8166e-03 \\ 
-4.0e+00 2.6688e-03 \\ 
-2.0e+00 4.7893e-04 \\ 
0.0e+00 6.1832e-03 \\ 
            }
            node [pos=.2,pin={[text=black,pin edge={text=black,solid,black,<-}]-90:$\Ma = 10$},inner sep=1pt] {};
            ;
        \addlegendentry{EP};

        \addplot [color=blue,dashed,line width=1.2pt,forget plot]
        table[row sep=crcr]{%
         -2.0e+01 1.5093e-01 \\ 
-1.8e+01 1.0327e-01 \\ 
-1.6e+01 6.9159e-02 \\ 
-1.4e+01 4.3282e-02 \\ 
-1.2e+01 2.3703e-02 \\ 
-1.0e+01 9.2590e-03 \\ 
-8.0e+00 2.7036e-03 \\ 
-6.0e+00 1.5654e-03 \\ 
-4.0e+00 2.4849e-03 \\ 
-2.0e+00 1.9982e-04 \\ 
0.0e+00 3.9117e-05 \\ 
            }
            ;
        % \addlegendentry{EP};

        \addplot [color=red,line width=1.2pt]
        table[row sep=crcr]{%
            -2.0e+01 7.5806e-02 \\ 
-1.8e+01 5.1502e-02 \\ 
-1.6e+01 3.4138e-02 \\ 
-1.4e+01 2.0243e-02 \\ 
-1.2e+01 1.0609e-02 \\ 
-1.0e+01 3.6786e-03 \\ 
-8.0e+00 5.8393e-04 \\ 
-6.0e+00 2.8144e-05 \\ 
-4.0e+00 1.7959e-06 \\ 
-2.0e+00 0.0000e+00 \\ 
0.0e+00 0.0000e+00 \\ 
            };
        \addlegendentry{AMP};

        \addplot [color=red,line width=1.2pt,forget plot]
        table[row sep=crcr]{%
            -2.0e+01 1.4809e-01 \\ 
-1.8e+01 1.0073e-01 \\ 
-1.6e+01 6.5473e-02 \\ 
-1.4e+01 4.1419e-02 \\ 
-1.2e+01 2.3201e-02 \\ 
-1.0e+01 8.0544e-03 \\ 
-8.0e+00 1.2944e-03 \\ 
-6.0e+00 8.5362e-05 \\ 
-4.0e+00 1.8431e-06 \\ 
-2.0e+00 1.8824e-06 \\ 
0.0e+00 0.0000e+00 \\ 
            }
            ;
        % \addlegendentry{AMP};

        \addplot [color=red,dashed,line width=1.2pt]
        table[row sep=crcr]{%
            -2.0e+01 7.5050e-02 \\ 
-1.8e+01 5.1050e-02 \\ 
-1.6e+01 3.3974e-02 \\ 
-1.4e+01 2.0221e-02 \\ 
-1.2e+01 1.0435e-02 \\ 
-1.0e+01 3.6992e-03 \\ 
-8.0e+00 5.5810e-04 \\ 
-6.0e+00 3.1063e-05 \\ 
-4.0e+00 1.7765e-06 \\ 
-2.0e+00 3.1429e-06 \\ 
0.0e+00 3.3765e-06 \\ 
            };
        \addlegendentry{scalar AMP};

        \addplot [color=red,dashed,line width=1.2pt,forget plot]
        table[row sep=crcr]{%
-2.0e+01 1.5853e-01 \\ 
-1.8e+01 1.0755e-01 \\ 
-1.6e+01 7.1402e-02 \\ 
-1.4e+01 4.8028e-02 \\ 
-1.2e+01 2.7266e-02 \\ 
-1.0e+01 1.1716e-02 \\ 
-8.0e+00 5.4950e-03 \\ 
-6.0e+00 4.6108e-03 \\ 
-4.0e+00 4.7200e-03 \\ 
-2.0e+00 3.2580e-03 \\ 
0.0e+00 3.6600e-03 \\ 
            }
            node [pos=.3,pin={[text=black,pin edge={solid,black,<-}]-0:$\Ma = 15$},inner sep=5pt] {};
            ;
        % \addlegendentry{scalar AMP};

        
      \end{semilogyaxis}
    \end{tikzpicture}
%     \vspace{-2mm}
% }
% \subcaptionbox{Wasserstein distance}[.5\textwidth][c]{
%     \begin{tikzpicture}
%     \tikzstyle{every node}=[font=\footnotesize] 
%     \begin{axis}[
%     scale only axis,
%     width=2.7in,
%     height=1.3in,
%     grid=both,
%     grid style={line width=.1pt, draw=gray!10},
%     major grid style={line width=.2pt,draw=gray!50},
% %scale only axis,
%     xmin=-20,
%     xmax=0,
%     xlabel={SNR (dB)},
%     ymin=.2,
%     ymax=.22,
%     % ymode = log,
%     ylabel={average Wasserstein distance},
%     ylabel style = {yshift=-1mm},
%      legend pos=south west,
%     ]
%        % \addplot [color=blue,line width=1.2pt]
%        %  table[row sep=crcr]{%
%        %      -10.000000000000000   0.208512049595293 \\
%        %    -8.000000000000000   0.206248911588813 \\
%        %    -6.000000000000000   0.203979471213634 \\
%        %    -4.000000000000000   0.203359891077836 \\
%        %    -2.000000000000000   0.202974915240486 \\
%        %                     0   0.203214737460965 \\
%        %     2.000000000000000   0.203120513664146 \\
%        %     4.000000000000000   0.203343859956285 \\
%        %     6.000000000000000   0.203090691968809 \\
%        %      };
%        %  \addlegendentry{$\Ma = 10$};

%         \addplot [color=blue,line width=1.2pt]
%         table[row sep=crcr]{%
%           -2.0e+01 2.1583e-01 \\ 
% -1.8e+01 2.1371e-01 \\ 
% -1.6e+01 2.0930e-01 \\ 
% -1.4e+01 2.0662e-01 \\ 
% -1.2e+01 2.0664e-01 \\ 
% -1.0e+01 2.0599e-01 \\ 
% -8.0e+00 2.0434e-01 \\ 
% -6.0e+00 2.0411e-01 \\ 
% -4.0e+00 2.0394e-01 \\ 
% -2.0e+00 2.0399e-01 \\ 
% 0.0e+00 2.0474e-01 \\   
%             };
%         \addlegendentry{EP};

%         \addplot [color=blue,dashed,line width=1.2pt,forget plot]
%         table[row sep=crcr]{%
%           -2.0e+01 2.1854e-01 \\ 
% -1.8e+01 2.1451e-01 \\ 
% -1.6e+01 2.1321e-01 \\ 
% -1.4e+01 2.1030e-01 \\ 
% -1.2e+01 2.0673e-01 \\ 
% -1.0e+01 2.0520e-01 \\ 
%-8.0e+00 2.0462e-01 \\ 
% -6.0e+00 2.0477e-01 \\ 
% -4.0e+00 2.0494e-01 \\ 
% -2.0e+00 2.0435e-01 \\ 
% 0.0e+00 0.0000e+00 \\ 
%             };
%         % \addlegendentry{EP};
        
%         \addplot [color=red,line width=1.2pt]
%         table[row sep=crcr]{%
%             -2.0e+01 2.1578e-01 \\ 
% -1.8e+01 2.1298e-01 \\ 
% -1.6e+01 2.1026e-01 \\ 
% -1.4e+01 2.0849e-01 \\ 
% -1.2e+01 2.0650e-01 \\ 
% -1.0e+01 2.0469e-01 \\ 
% -8.0e+00 2.0403e-01 \\ 
% -6.0e+00 2.0391e-01 \\ 
% -4.0e+00 2.0380e-01 \\ 
% -2.0e+00 2.0398e-01 \\ 
% 0.0e+00 2.0434e-01 \\ 
%             };
%         \addlegendentry{AMP};

%         \addplot [color=red,line width=1.2pt,forget plot]
%         table[row sep=crcr]{%
%             -2.0e+01 2.1895e-01 \\ 
% -1.8e+01 2.1493e-01 \\ 
% -1.6e+01 2.1299e-01 \\ 
% -1.4e+01 2.1047e-01 \\ 
% -1.2e+01 2.0819e-01 \\ 
% -1.0e+01 2.0558e-01 \\ 
% -8.0e+00 2.0468e-01 \\ 
% -6.0e+00 2.0463e-01 \\ 
% -4.0e+00 2.0483e-01 \\ 
% -2.0e+00 2.0461e-01 \\ 
% 0.0e+00 2.0429e-01 \\ 
%             };
%         % \addlegendentry{AMP};

%         \addplot [color=red,dashed,line width=1.2pt]
%         table[row sep=crcr]{%
%             -2.0e+01 2.1905e-01 \\ 
% -1.8e+01 2.1538e-01 \\ 
% -1.6e+01 2.1296e-01 \\ 
% -1.4e+01 2.1068e-01 \\ 
% -1.2e+01 2.0802e-01 \\ 
% -1.0e+01 2.0588e-01 \\ 
% -8.0e+00 2.0517e-01 \\ 
% -6.0e+00 2.0471e-01 \\ 
% -4.0e+00 2.0440e-01 \\ 
% -2.0e+00 2.0450e-01 \\ 
% 0.0e+00 2.0472e-01 \\ 
%             };
%         \addlegendentry{scalar AMP};

%         \addplot [color=red,dashed,line width=1.2pt,forget plot]
%         table[row sep=crcr]{%
%             -2.0e+01 2.1581e-01 \\ 
% -1.8e+01 2.1260e-01 \\ 
% -1.6e+01 2.1033e-01 \\ 
% -1.4e+01 2.0818e-01 \\ 
% -1.2e+01 2.0612e-01 \\ 
% -1.0e+01 2.0471e-01 \\ 
% -8.0e+00 2.0411e-01 \\ 
% -6.0e+00 2.0409e-01 \\ 
% -4.0e+00 2.0407e-01 \\ 
% -2.0e+00 2.0408e-01 \\ 
% 0.0e+00 2.0406e-01 \\ 
%             };
%         % \addlegendentry{scalar AMP};
%       \end{axis}
%     \end{tikzpicture}
%     \vspace{-2mm}
%     }

==> main.tex <==
% load all formatting options from my template 
\input{header-note}
%% -------------------------------------------------------------------------
%% cheat sheet 
%% new environments 
%% - marginfigure 
%% - margintable 
%% - fullwidth
%%
%% additional commands 
%% - todo 
%% ----------------------------------------------------------------------------
%%          Local commands 
%% Insert here local definitions 
%% ----------------------------------------------------------------------------
\author{Giuseppe Durisi}
\date{\today}
\title{Technical writing style guide}


\begin{document}

\maketitle
\tableofcontents
%
\newpage
%% ----------------------------------------------------------------------------
\section{Introduction}
%% ----------------------------------------------------------------------------
The purpose of this document is to identify a common writing style for the scientific
reports, publications, and  presentations, produced by the members of our team. We also
address recurring questions concerning grammar and spelling. Throughout, we assume the use
of \LaTeX. Recommendations that pertain publications in IEEE venues are highlighted with
the prefix (\emph{IEEE style}).

This document is heavily inspired by an excellent technical writing style guide produced
by Moritz Borgmann and Ulrich Schuster, two former colleagues of mine at the Communication
Theory Group, ETH, Zurich. Unfortunately, this guide is not available online, to the best
of my knowledge. It is also inspired by the excellent seminar series on paper writing lead
by my colleague Erik Agrell at Chalmers over the past few years.
The slides are available on the group intranet together with additional good material related to writing and publishing.\footnote{\url{https://wiki.portal.chalmers.se/s2/pmwiki.php/Comsys/WritingAndPublishing}}
The ``writing in science'' free course available on coursera is an excellent resource to improve your writing style.\footnote{Go to the \href{https://www.coursera.org/learn/sciwrite?utm_medium=sem&utm_source=gg&utm_campaign=b2c_emea_ibm-data-science_ibm_ftcof_professional-certificates_arte_feb_24_dr_geo-multi_pmax_gads_lg-all&campaignid=21041942377&adgroupid=&device=c&keyword=&matchtype=&network=x&devicemodel=&adposition=&creativeid=&hide_mobile_promo&gad_source=1&gclid=CjwKCAiA_tuuBhAUEiwAvxkgTmNteGZOQbJDn8s57tfSHyF4WU6LbA_7mo57sJvMlMPh8eWXspQpahoCH8oQAvD_BwE}{coursera link}}

\section{Style}
\subsection{Punctuation}
%
\begin{itemize}
	\item \textbf{Comma after introductory matter}: Most introductory matter at the beginning of
	      a sentence (be it adverbs, adverbial phrases, or dependent clauses) is followed by a
	      comma. Examples: \emph{``If you accept our conditions, we shall agree to the
		      proposal.'' ``After reading the note, Martha turned pale.'' ``In this context, we note that\dots''}
	\item \textbf{Conjunctive adverbs: thus, hence, therefore, etc\dots} Conjunctive adverbs at the beginning of
	      a sentence need to be separated by a comma in most cases. Example:
	      \emph{``Thus, we conclude that\dots''}
	      Note that conjunctive adverbs are not conjunctions, and should not be used to join
	      independent clauses. That is, do now write: ``\emph{We observed effect X, hence we
		      can conclude\dots''}. The correct punctuation mark in this case is a semicolon.
	      Conjunctive adverbs include: \emph{after all, in addition, next, also,
		      incidentally, nonetheless, as a result, indeed, on the contrary, besides, in fact,
		      on the other hand, consequently, in other words, otherwise, finally, instead, still,
		      for example, likewise, then, furthermore, meanwhile, therefore, hence, moreover, thus,
		      however, and nevertheless.}
	\item \textbf{Punctuation after displayed math}: The rule I typically follow is that
	      after displayed equations, the only punctuation allowed is a period.
	      Do not set a space between the equation and the punctuation. An alternative,
	      style, often required by some publications and followed by some authors, is
	      instead to punctuate after displayed equations as if the equation was part of the
	      text. This implies that commas and all other punctuation symbols are allowed.
	\item \textbf{Dashes}: The three main kinds of dashes are hyphen (-, yielding -), en
	      dashes (\verb|--|, yielding --), and em dashes (\verb|---|, yielding ---). One
	      uses em dashes to provide additional information that is not essential to
	      understand the sentence, similar to parentheses and commas. Example: ``\emph{Some
		      years ago---never mind how long precisely---I thought I would sail about a little
		      and see the watery part of the world.}'' They can also be used to mark a break in a
	      sentence, in place of a semicolon or a colon. Example: \emph{``There was no arguing
		      with her---she was set in her opinion''}. Note that em dashes should be set without
	      adjacent spaces.
	      Use en dashes to connect continuing or inclusive numbers. Example: write
	      \emph{Figs.~1--3} and not \emph{Figs.~1-3}.
	\item \textbf{I.e., e.g.}: Always set a comma after \emph{that is, namely, i.e., e.g.}
	\item \textbf{Ordinal numbers}: Write ``the $i$th entry'' instead of the ``the
	      $i$-th entry''.
	\item \textbf{Serial comma}: When a conjunction joins the last to elements in a
	      series, a comma should appear before the conjunction. Example: \emph{apples,
		      pears, and bananas.}
	\item \textbf{Large numbers}: Structure numbers larger than four digits by
	      separating group of three digits by a \verb|\medspace| (not a full space).
	      Example: write $\num{16777216}$ \emph{colors} instead of $16777216$ \emph{colors}.
	      Use the command \verb|\num{...}| of the package \verb|siunitx| to get the correct
	      layout automatically.
\end{itemize}
%
\subsection{Spelling}
%
\begin{itemize}
	\item \textbf{American English}: use American English spelling, not British English. For
	      example, write \emph{color} instead of \emph{colour}, \emph{capitalize} instead of
	      \emph{capitalise}, \emph{modeling} instead of \emph{modelling}.
	      Run a spell checker tool with an American English dictionary. Make sure to run the
	      spell checker tool before sending a paper draft to your
	      co-authors/collaborators/supervisors.
	\item \textbf{Contractions}: do not use contractions such as \emph{don't}, \emph{isn't},
	      etc\dots, in written language.
	\item \textbf{Headings}: (\emph{IEEE style}) use headline style for capitalizing the
	      first three levels of headings (i.e., sections, subsections, and subsubsections):
	      specifically, the first and last word and all nouns, pronouns, adjectives, verbs,
	      adverbs, and subordinating conjunctions (\emph{if, because, that, etc\dots}) are
	      capitalized. Articles, coordinating conjunctions (\emph{and, but, or, for, not}), and
	      prepositions, regardless of the length, are lowercased unless they are the first or
	      last word of the title. The \emph{to} in infinitives is also lowercased.
	      Use sentence-style capitalization for quaternary headings (i.e., paragraphs).
	\item \textbf{References to entities}: capitalize the entity name you refer to if you
	      mean a specific one. For example, write ``in Section~IV''.
	      However, write ``in the next section'' or ``in this section''.
	      Do not abbreviate Section, Chapter, Table, Appendix. However, write ``Fig.~3'' and
	      ``Figs. 1--3''.
	\item \textbf{References to equations:} use the \verb|\eqref{...}| command to refer to
	      equations. Say ``in (12)'' instead of ``in eq. (12)''.
	      However, do not begin a sentence with an equation reference number.
	      Instead, write for example ``Equation (12) concludes the proof''.
	\item \textbf{Prefixes:} Nearly all compounds words formed with prefixes are set
	      unhyphenated. Some prefixes are \emph{infra, inter, intra, macro, meta micro, mid,
		      min, multi, neo, non, over, post, pre, pro, proto, pseudo, re, semi, socio, sub,
		      super, supra, trans, ultra, un}, and \emph{under}.
	      For example, write \emph{noncoherent, multiantenna}, and \emph{pseudoinverse} (set all
	      of them unhyphenated).
	\item \textbf{Hyphenation of compound modifiers}: this is a tricky and controversial
	      issue. When compound modifiers (also called phrasal adjectives) appear later in a phrase
	      that the noun they describe, ambiguity is unlikely and the hyphen dispensable.
	      However, when such compounds precede a noun, hyphenation usually makes for easier
	      reading.
	      Examples: write ``\emph{this distribution is capacity achieving}'' but ``\emph{we found the
		      capacity-achieving distribution}''. Other examples: \emph{single-antenna communication,
		      information-theoretic results, frequency-division multiple-access systems}.
	\item \textbf{Hyphenation of special compounds}: write \emph{a $\qty{3}{dB}$ improvement, a
		      $10\%$ gain} (unhyphenated).
	\item \textbf{Acronyms}: use acronyms sparingly and introduce them at the first
	      occurrence (with the acronym in parenthesis). Do not capitalize the expression
	      defining the acronym, except if it is a trademarked expression. Examples: write
	      ``\emph{digital signal processor (DSP)'', Global System for Mobile Communications (GSM)}''.
	      Consider using the package \verb|glossaries| to keep track of all acronyms
	      introduced in the paper and make sure that they are defined only once.
\end{itemize}
%

\subsection{Typography}
%
\begin{itemize}
	\item \textbf{Use of italics and boldface}: use italics and boldface as sparingly as
	      possible. Use italics (\verb|\emph{...}|) for emphasizing words or short passages.
	      Do not use boldface for this purpose, as it destroys the uniform gray appearance
	      of the page.
	      Do not try to emulate sections or paragraphs using boldface.
	      Use the built-in commands, such as \verb|\subsections{...}| and
	      \verb|\paragraphs{...}|.
	\item \textbf{Underlined text:} Do not underline text. Underlining is a sensible
	      typographical option only in handwriting or manual typewriting, when italics letters
	      are not available.
	\item \textbf{Et al.}: Italicize \emph{et al.}; Also note that there is no period after
	      \emph{et} (which is not an abbreviation---it means ``and'' in latin).
	\item \textbf{Units}: unit symbols must be set upright, not italic. Set a
	      nonbreaking space between the number and the unit. Examples: $\qty{100}{Hz}$,
	      $\qty{50}{dB}$. Use the function \verb|\qty{...}{...}| from the \verb|siunitx|
	      package to get the correct layout automatically.
\end{itemize}
%
\subsection{Math}
%
\begin{itemize}
	\item \textbf{Ellipses:} use an ellipses (\verb|\ldots|) instead of three dots (...) in
	      an enumeration, to achieve a more regular spacing.
	      For example, write $n=1,2,\ldots,n$ instead of $n=1,2,..., n$.
	      Use centered dots (\verb|\cdots|) when omitting elements in a sum, product, or
	      (in)equality.
	      For example, write $a_{1}+a_{2}+\cdots+a_{n}$.
	      Also use $\cdots$ for omissions in vectors: $\veca = \tp{[a_{1} a_{2}\cdots a_{n}]}$.
	\item \textbf{Fractions:} in text, write $a/b$ instead of $\frac{a}{b}$.
	      When the math becomes ambiguous, use parentheses. For example, write $(a/b)c\sub{t}$.
	\item \textbf{Notation:} In a paper that is heavy in math, it is important to decide
	      whether it is worth distinguishing between scalars, vectors, and matrices, using
	      special fonts, and whether it is important to distinguish between random quantities
	      and their realizations.
	      Once this decision is made, it is good to inform the reader about it in the
	      introduction of the paper. It is also crucial to be consistent throughout the paper.
	      For an excellent and comprehensive example on how to write a math notation section, see, for
	      example~\cite[Section~II]{lapidoth03-10a}.
\end{itemize}
%
\subsection{References}
\subsubsection{Citations}
%
\begin{itemize}
	\item \textbf{Citations in abstract}: avoid citations in the abstract; if they are
	      necessary, do not use numerical citation style, but author-year citation style.
	      Examples: ``\emph{The proposed coding scheme is \qty{1}{dB} away from the converse
		      bound proposed in Polyanskiy et al. (2010).}
	\item \textbf{Citations to books:} always give section, page, etc\dots, when referring
	      to books. Do not expect the reader to go through the entire book to find evidence for
	      a claim in the paper.
\end{itemize}
%
\subsubsection{Bibliography}
\begin{itemize}
	\item \textbf{Journal and conference names}: use generally accepted abbreviations for
	      journal and conference names.
	      Make sure that you are consistent!
	      For conferences, do not include the year suffix, and
	      specify the place in which the conference took place. For books, specify the place in
	      which it was published. Here are some examples (\emph{IEEE style}):\footnote{For more
		      examples, please consult~\cite{shell15-08a}.}
	      %
	      \begin{itemize}
		      \item
		            Y.~Polyanskiy, H.~V. Poor, and S.~Verd\'u, ``Channel coding rate in the finite
		            blocklength regime,'' {\em {IEEE} Trans. Inf. Theory}, vol.~56,
		            pp.~2307--2359, May 2010.
		      \item
		            G.~Vazquez-Vilar, A.~Campo, A.~Guill\'en~i F\`abregas, and A.~Martinez, ``The
		            meta-converse bound is tight,'' in {\em Proc. IEEE Int. Symp. Inf. Theory
				            (ISIT)}, Istanbul, Turkey, pp.~1730--1733, July 2013.
		      \item
		            A.~Lapidoth, {\em A Foundation in Digital Communication}.
		            Cambridge, U.K.: Cambridge Univ. Press, 2009.
	      \end{itemize}
	      %
	      In general, make sure to follow the journal/conference's reference formats
	      (item ordering, capitalizing, italicizing, author names, journal abbreviations, month abbreviations, \dots).
	      Proofread carefully (author spelling and initials, spaces, commas, dashes, \dots)
	\item \emph{Electronic resources:} use the \verb|url| package to obtain sensible
	      linebreaks in long URLs.
	\item \emph{Familiarity with bibliography}: Read all your references (fully or at
	      least partially).
\end{itemize}
\subsection{Figures}
%
\begin{itemize}
	\item \textbf{Float placement:} When placing floats (figures and tables), avoid
	      specifying the positioning (specifically, the \verb|h| option).
	      Rely instead on the default placement, which will usually place the floats at the top
	      of the page.
	\item \textbf{Text in figures:} Sentence capitalization is recommended in all cases
	      where complete sentences are used in the figure. All incomplete sentences, like axes
	      labels, are set in lowercase.
	\item \textbf{Font size:} The font size should usually match the size of the captions.
	      This means that figures from Matlab/Python should not be directly imported into
	      two-column IEEE documents without proper resizing. My strong advice is to produce figures
	      using, instead the \verb|pgfplot| package.
	      Fig.~\ref{fig:good-fig}, whose \LaTeX code is available in the overleaf
	      repository, is produced using \verb|pgfplot|.
	\item \textbf{Caption:} use sentence capitalization; end figure caption with a period.
	\item \textbf{Legends and curves:} Avoid showing too many curves in a single plot.
	      The curves should have a sufficient line width and be well distinguishable by their
	      markers in black and white prints.
	      When possible, omit legends altogether and mark the curves directly by putting the
	      parameters with a little arrow next to the curve. See Fig.~\ref{fig:good-fig} for an
	      example of a good figure.
	      \begin{figure}[t]
		      \centering
		      \includegraphics[width=\textwidth]{./figs/results_u4_random.pdf}
		      \caption{An example of a good figure produced with pgfplot (the \LaTeX\, file is
			      in overleaf): EVM availability for $U = 4$ randomly positioned UEs. The dashed
			      line denotes the EVM availability for a co-located system in which a massive MIMO
			      base station with $64$ antennas serves all four UEs.}
		      \label{fig:good-fig}
	      \end{figure}
	\item \textbf{Titles:} the figure should have no title; move the information in the
	      caption instead.
	\item \textbf{Subfigures:} Label subfigures by (a), (b), (c), etc\dots Refer to
	      subfigures as, e.g., ``Fig. 3(a)''. Use the package \verb|subcaption|, to
	      automatize this process.
\end{itemize}
%
\subsection{Miscellaneous}
%
\begin{itemize}
	\item \textbf{Awkward line breaks:} Avoid awkward line breaks that put single
	      mathematical symbols, numbers, or references to section, figures, bibliographical
	      elements, and equations at the beginning of a new line. Use nonbreaking spaces
	      (\verb|~|) to keep \LaTeX\, from breaking a new line. For example always write
	      \verb|Fig.~\ref{...}| instead of \verb|Fig. \ref{...}|.  Avoid line
	      breaks in expressions such as ``by~$\matA$'', ``in~(3)'', ``in~[3]'', or `Fig.~3''.
	      Never start a sentence with math.
	\item \textbf{Footnote placements:} Footnotes should never be placed after math as this
	      may create ambiguity. For example do not write, ``\emph{we indicate this quantity as
		      $x$}\footnote{This footonote is misplaced; it may be interpreted as a mathematical
		      symbol.}''. Footnotes should be placed after punctuation. For example, write
	      ``\emph{the channel is assumed to be perfectly known at the receiver.\footnote{The
			      case of imperfect channel state information is discussed in Section~IV.}} Note
	      that the footnote is placed \emph{after} the period and not before it.
\end{itemize}
%
\section{Grammar}
%
\begin{itemize}
	\item \textbf{Relative clauses and commas:}  There is a distinction between relative clauses with and without preceeding comma.
	      %
	      \begin{itemize}
		      \item \emph{Defining (or restrictive) relative clauses}: the information provided in
		            a defining relative clause is crucial in understanding the meaning of the
		            sentence. Examples: \emph{``The woman who lives in apartment no.~34 has been
			            arrested''. ``The document that I need has important written at the top.''}
		            The purpose of a defining relative clause is to clearly define who or what we are
		            talking about. Without this information, it would be difficult to know who or what
		            is meant.
		      \item \emph{Nondefining (or nonrestrictive) relative clauses:} they provide
		            interesting additional information that is not essential to understand the meaning
		            of the sentence. Example: \emph{``Mrs. Jackson, who is very intelligent, lives on
			            the corner.''}
	      \end{itemize}
	      %
	      Correct punctuation is essential in nondefining relative clauses. If they occur in the
	      middle of a sentence, a comma is put before the relative pronoun and at the end of the
	      clause. If they occur at the end of the sentence, a comma is put before the relative
	      pronoun. In defining relative clauses, there are no commas.
	      The relative pronoun ``\emph{that}'' is typically used for defining relative clauses.
	      This means that there should be typically no comma before ``\emph{that}''.
	      The relative pronoun ``\emph{which}'' is typically used for nondefining relative clauses.
	      This means that there should be typically a comma before ``\emph{which}''.
	      The personal relative pronouns \emph{``who'', ``whose'', ``whom'',  ``where'',  ``when''}
	      can be used in both defining and nondefining clauses---the distinction is made by the
	      punctuation.
	\item \textbf{Elliptical construction:} Write ``\emph{the difference between the real-valued
		      case and the complex-valued case}'' instead of ``\emph{the difference between the real-valued
		      and the complex-valued case}''.
	\item \textbf{Either\dots or, neither\dots nor}: both constructions take a singular verb
	      when both the alternatives are singular or when the second alternative is singular.
	      In all other cases, a plural verb follows. Example: ``\emph{neither transmitter
		      nor receiver has CSI.}
\end{itemize}
%
\section{Usage}
%
\begin{itemize}
	\item \textbf{cf./see}: There is a clear distinction between the two: ``cf.'' originates
	      from the Latin ``\emph{conferre}'', which means ``compare''. This means that the
	      phrase ``cf. [1]'' is appropriate if the authors wish to point the reader to a
	      comparison between the point they have made and what reference [1] says. Comparison
	      may involve differences, similarities, or both. However, if the reference to which ``cf.''
	      points is merely meant as illustrative or corroborating, just say ``see [1]''. In
	      almost all cases, it is more appropriate to write ``see Section~I'', ``see [1]'', and
	      especially, ``see Table~1'' and ``see Fig.~1''.
	\item \textbf{Due to the fact that:} this phrase should almost always be replaced with
	      \emph{because} or any similar conjunction such as \emph{as}, \emph{for}, or
	      \emph{since}. \emph{Due to the fact that} is not wrong; it is just clumsy and
	      uneconomical.
	\item \textbf{Based on}: it can be used to carrying a verbal force (example: ``\emph{we
		      based our conclusion on measurements}'') or adjectival force (example: ``\emph{The
		      findings are based on measurements}''.
	      However, it should not have adverbial force, e.g., ``\emph{we arrived at our
		      conclusions based on measurements}'', or preposition force, e.g., ``\emph{based on our
		      measurements, we conjecture\dots}'', where \emph{based on} is now a dangler (see next
	      item).
	\item \textbf{Avoid danglers}: A dangler\footnote{Source: \url{https://grammarist.com/grammar/danglers/}} is a sentence element that does not relate
	      syntactically to the noun it is intended to modify. Danglers should be avoided since
	      they may create confusion, even if the reader may understand the intended meaning of
	      the sentence. Example of a dangler: ``\emph{Leaving home, the weather was sun and
		      crispy''}. The sentence is constructed as if to state that the weather is leaving
	      home, although we can guess that this is not the intention of the writer.
	      Here is another typical example to avoid in scientific writing:
	      ``\emph{Substituting (1) and
		      (2) into (3), the theorem is established}.'' Write instead: ``\emph{We establish the
		      theorem by substituting (1) and (2) into (3)}''.
\end{itemize}
%
\section{Structure}
A (journal) paper contains typically the following structural elements:
%
\begin{itemize}
	\item \textbf{Abstract}: The abstract should concisely describe (in one sentence) the main results of the paper.
	      It should not contain numbered references.
	      If references are necessary, they should be spelled out,
	      so that the abstract can always be read without access to the paper as a whole.
	      In the abstract, we should highlight what was found, not what was done. The abstract should not include
	      anything that is not said in the paper.
	\item \textbf{Index terms (IEEE)}: The index terms should be sorted alphabetically.
	      Acronyms should be listed together with their full definition.
	\item \textbf{Introduction}: The introduction should contain the following elements:
	      %
	      \begin{itemize}
		      \item A motivation for the proposed work.
		      \item A summary of relevant prior works, with knowledge gaps clearly identified.
		      \item A summary of the novel contributions made in the paper (preferably, as a
		            bullet point list).
		      \item An explanation of the notation used.
		      \item An outline of the paper: The outline should follow the logical steps presented
		            to arrive at the answers the questions outlined in the introduction.
		            A simple summary of section headings does not serve this purposes and may
		            be skipped.
	      \end{itemize}
	      %
	\item \textbf{Main sections} (numbered sections). A reasonably structured paper usually contains four to six main sections.
	\item \textbf{Conclusions}: The conclusion section should discuss the results
	      obtained in the paper and answer the question ``so what?''. Connections to prior
	      works can again be discussed. Open questions and future research questions can
	      also be addressed. The conclusion section should not be used to reiterate the main
	      findings reported in the paper and summarized in the abstract.
	\item \textbf{Appendices}, numbered with roman numbers or alphabetically: put there
	      proofs that would break the flow of the paper, because of their length and
	      technical nature.
	\item \textbf{Acknowledgements} (optional, unnumbered section): acknowledge, if
	      needed the contribution of fellow researchers that are not in the author list.
	\item \textbf{References} (unnumbered section).
	\item \textbf{Biographies} (\emph{IEEE style}, accepted manuscript).
\end{itemize}
%
\section{Presentations}
%
Excellent presentations require good planning and plenty of rehearsal.
So start early with your preparations.
Here are some recommendations.
\begin{itemize}
  \item \textbf{Before you start}: identify who the audience is and their
    level of expertise (what is the audience degree of familiarity with the topic you are
  going to present?); write down $1$ to $3$ take-home messages you want your audience to
  remember after your presentation.
\item \textbf{Prepare initial draft}: define the structure of
  the presentation (for example as a list of bullet points), from beginning to end; what needs to be mentioned when to deliver your
  main take-home messages? 
  This may take multiple iterations.
  Discuss this structure with your advisor, as well as the take-home messages.
\item \textbf{Slide preparations}: create one slide for each one of the items in your
  bullet point list; make sure that the total number of slides is compatible with the
  available time (a rule of thumb is to plan at least $\qty{90}{s}$). Prepare
  also a written script for each slide; it should more or less contain what you intend to
  say in each slide. What you write in the script should not necessarily appear in the
  slides. Think about the slides as containing useful material for your audience to follow
  what you are saying. Note that the slides should not be self contained (it requires
  someone to present them!). 
  This is the reason why you need to have a script, especially when rehearsing the presentation the first times! 
  When preparing the script, pay specific attention on what you are
  going to say on the first slide, the last slides, and the slides where you plan to
  deliver your take-home messages. 
  My suggestion is to simply memorize these parts and to use the rest of the script as
  inspiration for what you are going to say. 
  The last slides should contain your conclusions and take-home message, as well as a copy
  of one of the most representative figures in the presentation. This is the slide you
  want to keep on screen during the question \& answer session. Do not add any ``Thank
  you'' slide to your slide deck. 
\item \textbf{Rehearse:} rehearse your presentation multiple times. Adjust script and slide
  content to fulfill comfortably the time requirements. Record your presentation and
  listen to it, to double-check on pronunciation and intonation. Ask your team colleagues
  to attend one of your dry runs: are they able to identify the main take-home messages
  you intended to deliver?
\end{itemize}
\section{\LaTeX\, Intricacies}
%
\begin{itemize}
	\item \textbf{How to typeset equations in \LaTeX?}
	      What to do with equations that are too long? How to wrap them correctly?
	      The best solution involves the use of the environments \verb|multline| and
	      \verb|IEEEeqnarray| (for IEEE publications). In particular, \verb|IEEEeqnarray| should
	      should be used in any case instead of \verb|align| and \verb|eqnarray|. For more
	      information on how to typeset equations with \verb|multline| and  \verb|IEEEeqnarray|, read the excellent guide by Stefan
	      Moser.\footnote{Available at \url{https://moser-isi.ethz.ch/docs/typeset_equations.pdf}}
	\item \textbf{Operators}: Use operator commands to obtain the correct font and spacing.
	      For example, write
	      $y = \sin x$ instead of $y = sin x$.
	      If a certain operator does not exist, declare it.
	      Math operators can easily be declared using the
	      \texttt{AMS}-\LaTeX\, command \verb|\DeclareMathOperator{...}{...}|.
	\item \textbf{Semantic markup}:
	      A key rule to efficient and elegant \LaTeX ing is to write semantic, not visual,
	      markup. In other words, the focus of the bulk of the \LaTeX\, code should not be
	      on the appearance, but on the content. Whenever appearance needs to be defined,
	      this definition should be separated from the content as much as possible.
	      Following these rules usually leads to less error-prone code, faster typing, and
	      code that is easier to maintain and reuse.
	      In the following, this abstract advice shall be made more concrete.
	      \LaTeX's macro facilities serve as a key enabling tool for semantic markup.
	      For all (mathematical) entities that are used throughout a document,
	      define a macro, and use this macro instead of the written-out form. For example, define
	      \begin{verbatim}
          \newcommand{\Mt}{M_{\mathrm{t}}
        \end{verbatim}
	      and later on use \verb|$\Mt$| instead of the more awkward \verb|$M_{\mathrm{t}}$| to
	      write $M_{\mathrm{t}}$.
	      The advantage is threefold: the typing effort is reduced, errors are less likely,
	      and the notation can be easily changed later.
	      Macros can also take arguments. For example, the following definition may be
	      useful:
	      \begin{verbatim}
        \newcommand{\tp}[1]{\ensuremath{#1^{\mathrm{T}}}}
        \end{verbatim}
	      This command defines a transpose operator that can be used as follows:
	      \verb|$\tp{\mathbf{x}}$|, which yields $\tp{\mathbf{x}}$.
	      The two style files, named \verb|vmr-symbols-vecbold.sty| and \verb|standard-macros.sty|, which are included in the
	      overleaf repository,
	      contain a list of useful macros and operators that I use in all my papers.
	      To use them, include these two files in the preamble of your document via the
	      \verb|\usepackage{...}| command.
	      The best place to put these files is in the \url{/texmf/tex} folder of your latex
	      distribution.\footnote{This folder is typically in \url{~/Library/texmf/tex} on a MacOS.
		      In this way, these files become accessible globally on your machine.}
	\item \textbf{Operators followed by} \verb|\left| \textbf{and} \verb|\right| \textbf{delimiters}:
	      There is a very subtle spacing issue with variable-size delimiters: ordinary
	      delimiters, such as parentheses, are treated as math open atoms, whereas the
	      entire block enclosed by \verb|\left| and \verb|\right| is treated as math inner.
	      This has the sometimes undesired consequence that extra spacing is inserted before
	      the block.
	      This space is usually inappropriate when the opening delimiter follows an operator
	      (including sum and product signs), or when the delimiters denote the argument of a
	      function. To avoid this issue, our solution  is to define a new
	      variable-length delimiter, which we denote \verb|\lefto|, where the ``o'' stands for
	      operator, as follows
	      \begin{verbatim}
        \newcommand{\lefto}{\mathopen{}\left}
      \end{verbatim}
	      Note the difference in spacing between the this§ equation, in which we used
	      \verb|\lefto|
	      %
	      \begin{equation}
		      \log\det\lefto(1+ \frac{E\sub{s}}{N_{0}}\right) \prod_{i=1}^{N}\lefto(1+
		      \frac{a_{i}}{N}\right) f\lefto(\frac{x}{\abs{a}}\right)
	      \end{equation}
	      %
	      and this equation, where \verb|\left| is used and the spacing is incorrect
	      %
	      \begin{equation}
		      \log\det\left(1+ \frac{E\sub{s}}{N_{0}}\right) \prod_{i=1}^{N}\left(1+
		      \frac{a_{i}}{N}\right) f\left(\frac{x}{\abs{a}}\right).
	      \end{equation}
	      %
	\item \textbf{Line breaks:} Set your editor to use hard line breaks.
	      After intensive editing, the source code may  look ugly
	      (although modern text editors have commands for reformatting), hard breaks are
	      essential: most command-line tools like grep, less, more, diff, etc\dots are much
	      more useful when the length of lines is limited. Even more, most version control
	      systems (e.g., git) rely on hard line breaks for merging and diffing. Finally, if
	      you use reverse synchronization between your .tex editor and your pdf viewer, you
	      get much more precise synchronization if the length of the lines is short. This is
	      extremely useful when revising a paper.
  \item \textbf{Tools to prepare slides:} I recommend using the package  \verb|beamer| to
  prepare the slides, as it makes it simpler to copy math and figures directly from your
  scientific publications. It also forces you to be structured in terms of layout, which
  often leads to a more elegant and professional appearance.
  When using \verb|beamer|, set \verb|aspectratio=169|.
  Sometimes, it is convenient to have presentation notes. You can have them in
  \verb|beamer| as well by adding these commands 
  \begin{verbatim}
\usepackage{ifthen}
\newboolean{notes}
\setboolean{notes}{true}
% \setboolean{notes}{false}
\ifthenelse{\boolean{notes}}
{\setbeameroption{show notes on second screen=right}\nofiles}
{\setbeameroption{hide notes}}
  \end{verbatim}
 and then using the command \verb|\mynote|, which I defined as follows:
 \begin{verbatim}
 \newcommand{\mynote}[1]{\note[item]{\textbf{#1}}}  
\end{verbatim}
%
This command should be used on the slide you want to have presenter notes for.
To display the notes while presenting, you need a pdf viewer that is compatible with the
beamer dual-screen layout.
You may consider using \verb|pdfpc|\footnote{\url{https://pdfpc.github.io}}  or \verb|pympress|.\footnote{\url{https://github.com/Cimbali/pympress}}
Make sure that your laptop is \emph{not} in mirror mode.

\end{itemize}
%









\bibliographystyle{apalike2}
\bibliography{texxtracted}
% \bibliography{/Users/durisi/Library/texmf/bibtex/bib/personal/giubib.bib}
%% ----------------------------------------------------------------------------
\end{document}


==> preamble.tex <==
%\usepackage{amsmath,amssymb,eucal,amsthm}
%\usepackage{amsmath,amssymb,eucal}%,amsthm}
\usepackage{amsmath,amssymb,amsthm}
\usepackage{xifthen}
\usepackage{mathtools}
\usepackage{enumerate}
\usepackage{microtype}
\usepackage{xspace}
%\usepackage[noadjust]{cite}
\usepackage{bm}
\usepackage[T1]{fontenc}
%\usepackage[francais]{babel}
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage{bbm}


% vectors and matrices
%\newcommand{\mbs}[1]{\bm{#1}}
\newcommand{\mbs}[1]{\pmb{#1}}
\newcommand{\vect}[1]{{\lowercase{\mbs{#1}}}}
\newcommand{\mat}[1]{{\uppercase{\mbs{#1}}}}

\renewcommand{\Bmatrix}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\Pmatrix}[1]{\begin{pmatrix}#1\end{pmatrix}}

% transpose, hermitian transpose
\newcommand{\T}{{\scriptscriptstyle\mathsf{T}}}
\renewcommand{\H}{{\scriptscriptstyle\mathsf{H}}}
%\newcommand{\h}{{\scriptscriptstyle\mathsf{H}}}

\newcommand{\cond}{\,\vert\,}
\renewcommand{\Re}[1][]{\ifthenelse{\isempty{#1}}{\operatorname{Re}}{\operatorname{Re}\left(#1\right)}}
\renewcommand{\Im}[1][]{\ifthenelse{\isempty{#1}}{\operatorname{Im}}{\operatorname{Im}\left(#1\right)}}

\newcommand{\dotge}{\mathop{\dot{\ge}}}
\newcommand{\dotle}{\mathop{\dot{\le}}}

\newcommand{\mkv}{-\!\!\!\!\minuso\!\!\!\!-}

\newcommand{\SNR}{\mathsf{snr}}
\newcommand{\snr}{\mathsf{snr}}

\newcommand{\av}{\vect{a}}
\newcommand{\bv}{\vect{b}}
\newcommand{\cv}{\vect{c}}
\newcommand{\dv}{\vect{d}}
\newcommand{\ev}{\vect{e}}
\newcommand{\fv}{\vect{f}}
\newcommand{\gv}{\vect{g}}
\newcommand{\hv}{\vect{h}}
\newcommand{\iv}{\vect{i}}
\newcommand{\jv}{\vect{j}}
\newcommand{\kv}{\vect{k}}
\newcommand{\lv}{\vect{l}}
\newcommand{\mv}{\vect{m}}
\newcommand{\nv}{\vect{n}}
\newcommand{\ov}{\vect{o}}
\newcommand{\pv}{\vect{p}}
\newcommand{\qv}{\vect{q}}
\newcommand{\rv}{\vect{r}}
\newcommand{\sv}{\vect{s}}
\newcommand{\tv}{\vect{t}}
\newcommand{\uv}{\vect{u}}
\newcommand{\vv}{\vect{v}}
\newcommand{\wv}{\vect{w}}
\newcommand{\xv}{\vect{x}}
\newcommand{\yv}{\vect{y}}
\newcommand{\zv}{\vect{z}}
\newcommand{\zerov}{\vect{0}}

\newcommand{\nuv}{\vect{\nu}}
\newcommand{\muv}{\vect{\mu}}
\newcommand{\alphav}{\vect{\alpha}}
\newcommand{\betav}{\vect{\beta}}
\newcommand{\gammav}{\vect{\gamma}}
\newcommand{\deltav}{\vect{\delta}}
\newcommand{\phiv}{\vect{\phi}}
\newcommand{\Sigmam}{\pmb{\Sigma}}
\newcommand{\Lambdam}{\pmb{\Lambda}}
\newcommand{\Phim}{\pmb{\Phi}}
\newcommand{\Xim}{\pmb{\Xi}}
\newcommand{\Psim}{\pmb{\Psi}}
\newcommand{\Thetam}{\pmb{\Theta}}
\newcommand{\Omegam}{\pmb{\Omega}}

\newcommand{\Am}{\mat{a}}
\newcommand{\Bm}{\mat{b}}
\newcommand{\Cm}{\mat{c}}
\newcommand{\Dm}{\mat{d}}
\newcommand{\Em}{\mat{e}}
\newcommand{\Fm}{\mat{f}}
\newcommand{\Gm}{\mat{g}}
\newcommand{\Hm}{\mat{h}}
%\renewcommand{\Im}{\mat{i}}
\newcommand{\Jm}{\mat{j}}
\newcommand{\Km}{\mat{k}}
\newcommand{\Lm}{\mat{l}}
\newcommand{\Mm}{\mat{M}}
\newcommand{\Nm}{\mat{n}}
\newcommand{\Om}{\mat{o}}
\newcommand{\Pm}{\mat{p}}
\newcommand{\Qm}{\mat{q}}
\newcommand{\Rm}{\mat{r}}
\newcommand{\Sm}{\mat{s}}
\newcommand{\Tm}{\mat{t}}
\newcommand{\Um}{\mat{u}}
\newcommand{\Vm}{\mat{V}}
\newcommand{\Wm}{\mat{w}}
\newcommand{\Xm}{\mat{x}}
\newcommand{\Ym}{\mat{y}}
\newcommand{\Zm}{\mat{z}}

\newcommand{\AM}{\mat{a}}
\newcommand{\BM}{\mat{b}}
\newcommand{\CM}{\mat{c}}
\newcommand{\DM}{\mat{d}}
\newcommand{\EM}{\mat{e}}
\newcommand{\FM}{\mat{f}}
\newcommand{\GM}{\mat{g}}
\newcommand{\HM}{\mat{h}}
\newcommand{\IM}{\mat{i}}
\newcommand{\JM}{\mat{j}}
\newcommand{\KM}{\mat{k}}
\newcommand{\LM}{\mat{l}}
\newcommand{\MM}{\mat{M}}
\newcommand{\NM}{\mat{n}}
\newcommand{\OM}{\mat{o}}
\newcommand{\PM}{\mat{p}}
\newcommand{\QM}{\mat{q}}
\newcommand{\RM}{\mat{r}}
\newcommand{\SM}{\mat{s}}
\newcommand{\TM}{\mat{t}}
\newcommand{\UM}{\mat{u}}
\newcommand{\VM}{\mat{V}}
\newcommand{\WM}{\mat{w}}
\newcommand{\XM}{\mat{x}}
\newcommand{\yM}{\mat{y}}
\newcommand{\ZM}{\mat{z}}

% Calligraphic

\newcommand{\Ac}{{\mathcal A}}
\newcommand{\Bc}{{\mathcal B}}
\newcommand{\Cc}{{\mathcal C}}
\newcommand{\Dc}{{\mathcal D}}
\newcommand{\Ec}{{\mathcal E}}
\newcommand{\Fc}{{\mathcal F}}
\newcommand{\Gc}{{\mathcal G}}
\newcommand{\Hc}{{\mathcal H}}
\newcommand{\Ic}{{\mathcal I}}
\newcommand{\Jc}{{\mathcal J}}
\newcommand{\Kc}{{\mathcal K}}
\newcommand{\Lc}{{\mathcal L}}
\newcommand{\Mc}{{\mathcal M}}
\newcommand{\Nc}{{\mathcal N}}
\newcommand{\Oc}{{\mathcal O}}
\newcommand{\Pc}{{\mathcal P}}
\newcommand{\Qc}{{\mathcal Q}}
\newcommand{\Rc}{{\mathcal R}}
\newcommand{\Sc}{{\mathcal S}}
\newcommand{\Tc}{{\mathcal T}}
\newcommand{\Uc}{{\mathcal U}}
\newcommand{\Wc}{{\mathcal W}}
\newcommand{\Vc}{{\mathcal V}}
\newcommand{\Xc}{{\mathcal X}}
\newcommand{\Yc}{{\mathcal Y}}
\newcommand{\Zc}{{\mathcal Z}}


\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\RR}{\mathbb{R}}

\newcommand{\Id}{\mat{\mathrm{I}}}
\newcommand{\one}{\mat{\mathrm{1}}}

\newcommand{\CN}[1][]{\ifthenelse{\isempty{#1}}{\mathcal{N}_{\mathbb{C}}}{\mathcal{N}_{\mathbb{C}}\left(#1\right)}}

\renewcommand{\P}[1][]{\ifthenelse{\isempty{#1}}{\mathbb{P}}{\mathbb{P}\left(#1\right)}}
\newcommand{\E}[1][]{\ifthenelse{\isempty{#1}}{\mathbb{E}}{\mathbb{E}\left[#1\right]}}
\newcommand{\I}[1][]{\ifthenelse{\isempty{#1}}{\mathbb{I}}{\mathbb{I}\left\{#1\right\}}}
\renewcommand{\det}[1][]{\ifthenelse{\isempty{#1}}{\mathrm{det}}{{\rm det}\left(#1\right)}}
\newcommand{\trace}[1][]{\ifthenelse{\isempty{#1}}{{\rm tr}}{{\rm tr}\left\{#1\right\}}}
\newcommand{\rank}[1][]{\ifthenelse{\isempty{#1}}{\mathrm{rank}}{{\rm rank}\left(#1\right)}}
\newcommand{\diag}[1][]{\ifthenelse{\isempty{#1}}{\mathrm{diag}}{{\rm diag}\left(#1\right)}}
\newcommand{\Cov}[1][]{\ifthenelse{\isempty{#1}}{\mathsf{Cov}}{\mathsf{Cov}\left(#1\right)}}


\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclarePairedDelimiter\normf{\lVert}{\rVert_{\text{F}}}

\DeclareMathOperator{\arccot}{arccot}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Theorem, Definition, ...
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\defeq}{\triangleq}
\newcommand{\eqdef}{\triangleq}

\newtheorem{proposition}{Proposition}%[section]
\newtheorem{property}{Property}%[section]
\newtheorem{remark}{Remark}%[section]
\newtheorem{definition}{Definition}%[section]
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{example}{Example}%[section]
\newtheorem{corollary}{Corollary}%[section]
\newtheorem{conjecture}{Conjecture}%[section]
\newtheorem{fact}{Fact}%[section]
\newtheorem{lemma}{Lemma}%[section]
\newtheorem{assumption}{Assumption}%[section]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Answer & Solution
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{enumi_saved}
\setcounter{enumi_saved}{0}

\newenvironment{question}
{
\begin{enumerate}[Q1.]
    \setcounter{enumi}{\value{enumi_saved}}
}
{
\setcounter{enumi_saved}{\value{enumi}}
\end{enumerate}
}


\usepackage{answers}
\Newassociation{solution}{Solution}{solutionfile}
\renewcommand{\solutionextension}{sln}
\renewcommand{\Solutionparams}{{ Q\Currentlabel.}}
\renewcommand{\solutionstyle}[1]{#1}
\AtBeginDocument{\Opensolutionfile{solutionfile}[\jobname]}
\AtEndDocument{\Closesolutionfile{solutionfile}\clearpage
%\section*{Solutions}%
%\pagestyle{empty}\input{\jobname.sln}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Really Optional
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\IfFileExists{MinionPro.sty}{
%\usepackage{MnSymbol}
%\usepackage[mathlf,textlf,minionint]{MinionPro}
}{
%\usepackage[sc]{mathpazo}
%\linespread{1.05}         % Palatino needs more leading (space between lines)
}

%\mathtoolsset{showonlyrefs}





